R-NeRF: Neural Radiance Fields for Modeling RIS-enabled Wireless Environments

Recently, ray tracing has gained renewed interest with the advent of Reflective Intelligent Surfaces (RIS) technology, a key enabler of 6G wireless communications due to its capability of intelligent manipulation of electromagnetic waves. However, accurately modeling RIS-enabled wireless environments poses significant challenges due to the complex variations caused by various environmental factors and the mobility of RISs. In this paper, we propose a novel modeling approach using Neural Radiance Fields (NeRF) to characterize the dynamics of electromagnetic fields in such environments. Our method utilizes NeRF-based ray tracing to intuitively capture and visualize the complex dynamics of signal propagation, effectively modeling the complete signal pathways from the transmitter to the RIS, and from the RIS to the receiver. This two-stage process accurately characterizes multiple complex transmission paths, enhancing our understanding of signal behavior in real-world scenarios. Our approach predicts the signal field for any specified RIS placement and receiver location, facilitating efficient RIS deployment. Experimental evaluations using both simulated and real-world data validate the significant benefits of our methodology.

==> tables/4benchmarks.tex <==
% Table generated by Excel2LaTeX from sheet '对比实验'
\begin{table}
  \centering
  \caption{Received signal strength from various methods}
  \resizebox{0.45\textwidth}{!}{
   %\setlength{\tabcolsep}{4mm}{
    \begin{tabular}{cccc}
    \toprule
    
        %\multicolumn{2}{c}{ Methods} & \makecell[c]{Simulation data \\ (dBm)}   &\makecell[c]{Measured data \\ (dBm)}  \\
        & Methods & \makecell[c]{Simulation result \\ (dBm)}   &\makecell[c]{Measured result \\ (dBm)}  \\
        \midrule
            %zero  & -27.18  & -30.40  \\
            
            \multirow{3}[0]{*}{Model-based} 
                & APX \cite{zhang2022configuringAPX}  & -23.93  & -29.40  \\
                & SDR \cite{wu2019intelligentSDR}  & -23.89  & -29.24  \\
                & Manopt \cite{xiong2023risMAN}  & -23.80 & -29.27 
                \\
                \midrule
            \multirow{2}[0]{*}{Learning-based}
                & DNN \cite{huang2019indoor} & -20.28  & -28.85  \\
                & \textbf{Ours}  & \textbf{-16.85} & \textbf{-26.43} \\
    \bottomrule
    \end{tabular}%
    }
    %}
    \label{tab:Comparison experiments}%
\end{table}

==> tables/Network_Structure_Comparison.tex <==
\begin{table}
  \centering
  \caption{Network Structure Comparison}
 % \setlength{\tabcolsep}{1mm}%调整列宽
    \begin{tabular}{lcccc}
    \midrule
    \multirow{1}[2]{*}[0pt]{Network Structure}  & \multirow{1}[2]{*}[0pt]{MAE}  & \multirow{1}[2]{*}[0pt]{MED}& \multirow{1}[2]{*}[0pt]{RMSE}\\
    \midrule
    \multirow{1}{*}{Dual network RIS rendering} &1.58  & 1.10  &1.43\\ 
    \multirow{1}{*}{Dual network Rx rendering} &1.98  & 1.23 & 2.97 \\
    \multirow{1}{*}{Single network RIS rendering} &0.85  & 0.54  &1.19\\ 
    \multirow{1}{*}{Single network Rx rendering} &0.94  & 0.62  &1.37\\ 
    \multirow{1}{*}{Ours} &0.59  & 0.47  &0.78\\ 
    \midrule
    \end{tabular}%
  %\label{tab:ablation study}%
  \vspace{-0.4cm}
\end{table}%

==> tables/T1_ablation.tex <==
\begin{table}
  \centering
  \caption{Ablation experiments}
 % \setlength{\tabcolsep}{1mm}%调整列宽
    \begin{tabular}{cccccc}
    \toprule
    \multirow{2}[2]{*}[0pt]{Activation} & \multirow{2}[2]{*}[0pt]{PE} & \multicolumn{2}{c}{Simulation data} & \multicolumn{2}{c}{Measured Data} \\
    \cmidrule(r){3-4} \cmidrule(r){5-6}
         &       & enc   & w/o enc & enc   & w/o enc \\
    \midrule
    \multirow{2}[1]{*}{ReLU} & \ding{55} & 74.33\% & 58.37\% & 65.43\% & 56.42\% \\
                             & \ding{51} & \textbf{91.46\%} & 87.06\% & \textbf{70.94\%} & 64.41\% \\
    \midrule
    \multirow{2}[0]{*}{LeakyReLU} & \ding{55} &74.26\% & 58.30\% & 67.56\% & 59.13\% \\
                            & \ding{51} & 90.77\% & 87.58\% & 68.97\% & 63.64\% \\
    \midrule
    \multirow{2}[1]{*}{GELU} & \ding{55} & 74.40\% & 61.38\% & 65.98\% & 56.45\% \\
                             & \ding{51} & 90.88\% & 87.36\% & 69.94\% & 60.84\% \\
    \midrule
    \multirow{2}[0]{*}{Sin} & \ding{55} & 72.06\% & 54.66\% & 56.37\% & 52.84\% \\
                             & \ding{51} & 88.81\% & 83.62\% & 57.24\% & 53.19\% \\   
    \midrule
    \multirow{2}[0]{*}{Tanh} & \ding{55} & 74.33\% & 57.60\% & 64.75\% & 59.91\% \\
                                  & \ding{51} & 89.70\% & 86.85\% & 68.62\% & 61.79\% \\
       \bottomrule
    \end{tabular}%
  \label{tab:ablation study}%
\end{table}%
\vspace{-5pt}

==> tables/TheNeRF3prosss.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{l}
         \hline
         Alogrithm 1 The NeRF3 prosss \\
         \hline 
         \textbf{Input}： Position information $P_{tx}$、$P_{ris}$、$P_{rx}$ \\
         \textbf{Output}： Optimum Received Signal Strength $R_{best}$ \\
         1: Setting the number of sampled rays and the corresponding\\ \quad number of sampled voxels $M$、$N$\\
         2：Obtain information about the origin $r_o$ and direction $r_d$ of\\ \quad light  for $P_{ris}$、$P_{rx}$ respectively \\
         3: Calculate the voxel position information $P_v$ corresponding to\\ 
         \quad the light\\
         4: Constructing Position Encoding Functions $\gamma_{(emb)}$ and encode \\ \quad the position of the input information\\
         5: Setting MLP Network Parameters\\
         6：input the position-encoded information into the MLP network\\ \quad to obtain the rendering parameters\\
         7: Calculation of the received intensity according to the rendering\\ \quad equation $R_s$\\
         8：Complete network training optimization to predict optimal \\ \quad reception strength $R_{best}$\\
         \hline
    \end{tabular}
\end{table}

==> tables/TheR-NeRFprocess.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{l}
         \hline
         \textbf{Algorithm 1: The R-NeRF Method} \\
         \hline 
         \textbf{Input}: Position information $\mathbf{P_{TX}}$, $\mathbf{P_{RIS}}$, $\mathbf{P_{RX}}$ \\
         \textbf{Output}: Predicted signal strength at the receiver's location $\hat{R}_i$ \\
         1: Initialize the sampled ray direction information $d$; \\
         2: Set the number of sampled rays and voxels, $M$ and $N$ respectively; \\
         3: Sample $N$ voxel positions $\mathbf{P_v}$ using Eq. \eqref{eq:ray tracing}; \\
         4: Apply positional encoding (PE) to voxel positions $\mathbf{P_v}$, ray direction \\ \quad information $d$, $\mathbf{P_{TX}}$, and $\mathbf{P_{RIS}}$, using Eq. \eqref{eq:position encoding}, and feed them into \\ \quad the TN and RN network; \\
         5: Configure the parameters of the neural network as specified in Table I; \\
         6: Obtain the rendering parameters for the two stages: $S(\mathbf{P_{v_1}},\mathbf{d}_1)$, \\ \quad $T(\mathbf{P_{v_1}})$, $S(\mathbf{P_{v_2}},\mathbf{d}_2)$, $T(\mathbf{P_{v_2}})$; \\
         7: Calculate the predicted signal $\hat{R}_i$ using the rendering equations \\ \quad with Eq. \eqref{eq:R_total}, \eqref{eq:TX-RIS}, \eqref{eq:RIS-RX}; \\
         8: Optimize the neural network through the loss function of Eq. \eqref{eq:loss function}; \\
         9: Utilize the trained neural network model to predict the signal strength \\ \quad for unseen data. \\
         \hline
    \end{tabular}
    \vspace{-0.4cm}
\end{table}




==> tables/mlp_parameters.tex <==
% Table generated by Excel2LaTeX from sheet '网络参数'
\begin{table}
  \centering
  \caption{Key Network Parameters}
    \begin{tabular}{l|l}
    \hline
    \textbf{Parameter} & \textbf{Value} \\
    \hline
    Base frequency  & $C=1.35 $ \\
    Length of PE & $L=40 $ \\
    Dimension of input   & $6\times L$ \\
    Number of hidden layer & $L_h=4$ \\
    width of hidden layer  & $W_h=128$ \\
    optimizer & SGD \\
    Batchsize & $\text{Batchsize}=64$ \\
    Learning rate & $10^{-3}$ \\
    \hline
    \end{tabular}%
  \label{tab:parameters}%
\end{table}%
